Bayesian Nonparametric Sensitivity Analysis for Unmeasured Confounding in Data Fusion

Causal conclusions from observational data rest on assumptions, such as exchangeability over treatment, that cannot be verified from the data alone. Sensitivity analysis asks how conclusions change as such assumptions are relaxed. We develop a Bayesian nonparametric sensitivity analysis framework based on Causal-ICM, a multi-task Gaussian process model that places a prior on the causal response surface and the observational outcome regression. Their prior correlation is the key sensitivity parameter, where each value returns a full posterior for the average treatment effect, rather than only a bound or a point estimate. The framework applies to observational data alone and extends directly to settings where a randomised trial is available alongside a larger, potentially confounded observational study. Full pooling and the trial-only analysis then emerge as endpoints of the same sensitivity analysis. The posterior mean of the average treatment effect decomposes into a trial-only component plus a shift due to observational data, and for any correlation below one, posterior uncertainty remains bounded away from zero however large the observational study becomes. We illustrate the framework with simulations and a synthetic-data example combining a randomised trial of oral semaglutide with real-world health data, in which the trial's conclusion holds across the entire sensitivity range, regardless of how much the observational data are trusted.

==> latexmkrc <==
# Lets main_text.tex and supplementary.tex reference each other's labels (xr-hyper).
# When one document is compiled, the other is compiled first so that its .aux file exists.
# XR_NESTED stops the two documents from triggering each other in an endless loop.
add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');
sub makeexternaldocument {
    if (!($root_filename eq $_[0]) && !$ENV{XR_NESTED}) {
        local $ENV{XR_NESTED} = 1;
        system("latexmk -cd -pdf \"$_[0]\"");
    }
}


==> preamble_shared.tex <==
% Shared preamble for main_text.tex and supplementary.tex.
% Edit packages, macros, acronyms and the title/running head here once; both documents pick it up.
% xr-hyper must be loaded before hyperref: it lets each document \ref labels defined in the other.
\usepackage{xr-hyper}
\usepackage[margin=1in]{geometry}
\usepackage{setspace}
\doublespacing
% Encoding
\usepackage[utf8]{inputenc}
\usepackage{tikz} % Required for drawing graphics


\usepackage{multicol}
\usepackage{caption} % Required for \captionof
\usepackage{subcaption}
\usepackage[inline]{enumitem}

% Math packages
\usepackage{amsmath, amssymb, mathtools, amsthm, bbm}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\iid}{\overset{\mathrm{iid}}{\sim}}


% Theorem environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
%\theoremstyle{remark}
%\newtheorem{remark}[theorem]{Remark}


% TikZ and graphics
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{circuitikz}
\usepackage{pgf}
\usetikzlibrary{
  arrows, shapes.arrows, shapes.geometric,
  shapes.multipart, decorations.pathmorphing,
  positioning, swigs
}

% Comments and text highlighting
\usepackage[dvipsnames]{xcolor}
\newcommand{\edwin}[1]{{\textcolor{purple}{{(Edwin:} #1)}}}
\newcommand{\karla}[1]{{\textcolor{red}{{\bf(Karla:} #1)}}}
\newcommand{\evan}[1]{{\textcolor{ForestGreen}{{\bf(Evangelos:} #1)}}}
\newcommand{\brieuc}[1]{{\textcolor{cyan}{{\bf(Brieuc:} #1)}}}

% Miscellaneous
\setlength\parindent{0pt}
\usepackage[normalem]{ulem}  % underline without italics
\usepackage{algpseudocode}
\usepackage{url}
\usepackage{booktabs}
\usepackage{hyperref}
\usepackage{comment}
\usepackage{ytableau}
\ytableausetup{centertableaux}
\usepackage{tkzexample}
\usepackage{enumitem}

% Bibliography: APA author-date style via biblatex/biber.
% - style=apa: author-date citations, alphabetised reference list by first author's surname.
% - natbib=true: keeps the \citep/\citet syntax already used throughout the manuscript.
% - maxcitenames=3, mincitenames=1: in-text citations with <=3 authors give all authors on
%   the first citation, then collapse to the first author + et al.; 4+ authors always et al.
% - maxbibnames=6, minbibnames=6: reference-list entries with more than six authors list
%   the first six followed by et al.
\usepackage[style=apa, backend=biber, natbib=true, maxcitenames=3, mincitenames=1, maxbibnames=6, minbibnames=6, uniquename=false, uniquelist=false]{biblatex}
\addbibresource{bibliography.bib}


% Independence symbol
\newcommand\independent{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\usepackage{xcolor}
\newcommand{\ed}[1]{{\color{blue}#1}}

% Euler macro
\DeclareRobustCommand{\euler}{\genfrac<>{0pt}{}}

% Glossaries 
\usepackage{glossaries}
\newacronym{rct}{RCT}{randomised controlled trial}
\newacronym{gp}{GP}{Gaussian process}
\newacronym{hte}{HTE}{heterogeneous treatment effect}
\newacronym{ate}{ATE}{Average Treatment Effect}
\newacronym{cate}{CATE}{conditional average treatment effect}
\newacronym{icm}{ICM}{Intrinsic Coregionalization Model}
\newacronym{rwd}{RWD}{Real-World Data}
\newacronym{cf}{CF}{Causal Forest}
\newacronym{rf}{RF}{Random Forest}
\newacronym{rmse}{RMSE}{Root Mean Squared Error}
\newacronym{rlm}{RLM}{Random Location Model}
\newacronym{osm}{OSM}{Outcome Sensitivity Model}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\theoremstyle{plain}


% Title page and running head
\newcommand{\papertitle}{Bayesian Nonparametric Sensitivity Analysis for Unmeasured Confounding in Data Fusion}
\title{\papertitle}
\author{Evangelos Dimitriou}
% \date{June 2025}

% Running head: must be 50 characters or less (including spaces).
% Suggestion (45 characters): Bayesian Sensitivity Analysis and Data Fusion
\newcommand{\runninghead}{BNP Sensitivity Analysis to Unmeasured Confounding}

\usepackage{fancyhdr}
\pagestyle{fancy}
\fancyhf{}
\lhead{\small\runninghead}
\rhead{\small\thepage}
\renewcommand{\headrulewidth}{0pt}
\setlength{\headheight}{15pt}

% Cross-document references (xr-hyper). Works on Overleaf together with the latexmkrc file,
% which compiles the other document first so that its .aux file is available.
\makeatletter
\newcommand*{\addFileDependency}[1]{%
  \typeout{(#1)}%
  \@addtofilelist{#1}%
  \IfFileExists{#1}{}{\typeout{No file #1.}}%
}
\makeatother
\newcommand*{\myexternaldocument}[2]{%
  \externaldocument{#1}[#2]%
  \addFileDependency{#1.tex}%
  \addFileDependency{#1.aux}%
}

